Improving Design of Input Condition Invariant Speech Enhancement

Building a single universal speech enhancement (SE) system that can handle arbitrary input is a demanded but underexplored research topic. Towards this ultimate goal, one direction is to build a single model that handles diverse audio duration, sampling frequencies, and microphone variations in noisy and reverberant scenarios, which we define here as "input condition invariant SE". Such a model was recently proposed showing promising performance; however, its multi-channel performance degraded severely in real conditions. In this paper we propose novel architectures to improve the input condition invariant SE model so that performance in simulated conditions remains competitive while real condition degradation is much mitigated. For this purpose, we redesign the key components that comprise such a system. First, we identify that the channel-modeling module's generalization to unseen scenarios can be sub-optimal and redesign this module. We further introduce a two-stage training strategy to enhance training efficiency. Second, we propose two novel dual-path time-frequency blocks, demonstrating superior performance with fewer parameters and computational costs compared to the existing method. All proposals combined, experiments on various public datasets validate the efficacy of the proposed model, with significantly improved performance on real conditions. Recipe with full model details is released at https://github.com/espnet/espnet.

==> table/chime4.tex <==
\begin{table*}
    \setstretch{0.9}
    \caption{Experiments on the proposed methods trained and evaluated using the CHiME-4 (5ch) dataset. 
    Models are trained only on 8 kHz data, and tested on 16 kHz data. 
    The values within parentheses denote single-channel performance while all others are multi-channel performance.
    % All results are by default obtained based on multi-channel processing, while the number in parentheses denotes the corresponding result obtained based on single-channel processing. 
    The best and second best results are made bold and \underline{underlined}. All models except for Nos. 1 and 2 are our novel explorations.}
    \label{tab:exp_chime4}
    \centering
    % reduce the distance between columns in a table
    \setlength{\tabcolsep}{3pt}
    \resizebox{\textwidth}{!}{%
    \begin{tabular}{llccc|ccccc|cc}
        \toprule
        \multirow{2}{*}{\textbf{No.}} & \multirow{2}{*}{\textbf{Model}} & \multirow{2}{*}{\textbf{\#Param}} & \multicolumn{2}{c|}{\textbf{\#MAC (G/s)}} & \multicolumn{5}{c|}{\textbf{Test (CHiME-4 Simu)}} & \multicolumn{2}{c}{\textbf{Test (CHiME-4 Real)}} \\
        & & & \textbf{1ch} & \textbf{2ch} & \textbf{PESQ-WB} $\uparrow$ & \textbf{STOI ($\times100$)} $\uparrow$ & \textbf{SDR (dB)} $\uparrow$ & \textbf{DNSMOS OVRL} $\uparrow$ & \textbf{WER (\%)} $\downarrow$ & \textbf{DNSMOS OVRL} $\uparrow$ & \textbf{WER (\%)} $\downarrow$ \\
        \hline
        1 & No processing & - & - & - & 1.07 & 67.4 & -0.7 & 1.30 & 28.3 & 1.46 & \textbf{6.7} \\
        2 & USES ({\em baseline})~\cite{Toward-Zhang2023} & 3.05 M & 65.3 & 98.0 & \underline{3.16} & \underline{98.3} & 20.6 & \underline{3.22} & 4.2 & 1.99 (2.94) & 78.1 (11.0) \\
        \hline
        3 & w/ {\hypersetup{hidelinks}\hyperlink{symbol:decoupled_design}{decoupled}} proc. & 3.05 M & 60.8 & 98.0 & 2.62 & 97.0 & 18.2 & 3.08 & 5.2 & 2.32 & 27.8 \\
        4 & No.3 + 2-stage training & 3.05 M & 60.8 & 98.0 & 2.23 & 94.9 & 15.6 & 2.99 & 6.8 & 2.41 & 23.8 \\
        5 & No.3 + Att$\times1$ + \mathsymbol{TAC}$\times2$ & 3.02 M & 60.8 & 97.5 & \textbf{3.21} & \textbf{98.5} & \textbf{22.2} & 3.20 & \textbf{4.0} & 1.48 & 99.0 \\
        6 & No.5 + 2-stage training & 3.02 M & 60.8 & 97.5 & 2.98 & 97.9 & 19.0 & \underline{3.22} & 4.4 & 1.58 & 93.8 \\
        7 & No.3 +  {\hypersetup{hidelinks}\hyperlink{symbol:TAttC}{TA$_{\text{tt}}$C}}$\times3$ & 3.47 M & 60.8 & 116.9 & 2.72 & 97.3 & 18.7 & 3.14 & 5.2 & 2.40 & 28.8 \\
        8 & No.7 + 2-stage training & 3.47 M & 60.8 & 116.9 & 3.06 & 98.2 & 19.8 & 3.21 & 4.2 & 2.40 & 54.3 \\
        \hline
        9 & \mathsymbol{USES2-Swin} ({\em proposed}) & 2.92 M & 37.7 & 75.5 & 2.94 & 98.1 & 20.6 & 3.21 & 4.2 & 2.84 & 22.1 \\
        10 & No.9 + 2-stage training & 2.92 M  & 37.7 & 75.5 & 2.98 & 98.2 & \underline{21.1} & \underline{3.22} & \underline{4.1} & 2.80 & 24.9 \\
        11 & \mathsymbol{USES2-Comp} ({\em proposed}) & 2.53 M & 52.4 & 83.0 & 3.05 & \underline{98.3} & 20.4 & 3.21 & 4.2 & \underline{2.89} & 15.6 \\
        12 & No.11 + 2-stage training & 2.53 M & 52.4 & 83.0 & 2.94 & 97.9 & 18.8 & \textbf{3.23} & 4.6 & \textbf{2.96} & \underline{12.1} \\
%                \multirow{2}{*}{\textbf{No.}} & \multirow{2}{*}{\textbf{Model}} & \multirow{2}{*}{\textbf{\#Param}} & \multicolumn{5}{c|}{\textbf{Test (Simu)}} & \multicolumn{2}{c}{\textbf{Test (Real)}} \\
%        & & & \textbf{PESQ-WB} $\uparrow$ & \textbf{STOI ($\times100$)} $\uparrow$ & \textbf{SDR (dB)} $\uparrow$ & \textbf{DNSMOS OVRL} $\uparrow$ & \textbf{WER (\%)} $\downarrow$ & \textbf{DNSMOS OVRL} $\uparrow$ & \textbf{WER (\%)} $\downarrow$ \\
%        \hline
%        1 & No processing & - & 1.07 & 67.4 & -0.7 & 1.30 & 28.3 & 1.46 & \textbf{6.7} \\
%        2 & USES~\cite{Toward-Zhang2023} & 3.05 M & \underline{3.16} & \underline{98.3} & 20.6 & 3.22 & 4.2 & 1.99 (2.94) & 78.1 (11.0) \\
%        \hline
%        3 & w/ decoupled proc. & 3.05 M & 2.62 & 97.0 & 18.2 & 3.08 & 5.2 & 2.32 & 27.8 \\
%        4 & $\quad$+ 2-stage training & 3.05 M & 2.23 & 94.9 & 15.6 & 2.99 & 6.8 & 2.41 & 23.8 \\
%        5 & $\quad\rightarrow$ Att + TAC$\times2$ & 3.02 M & \textbf{3.21} & \textbf{98.5} & \textbf{22.2} & 3.20 & \textbf{4.0} & 1.48 & 99.0 \\
%        6 & $\qquad$+ 2-stage training & 3.02 M & 2.98 & 97.9 & 19.0 & 3.22 & 4.4 & 1.58 & 93.8 \\
%        7 & $\quad\rightarrow$ {\hypersetup{hidelinks}\hyperlink{symbol:TAttC}{TA$_{\text{tt}}$C}}$\times3$ & 3.47 M & 2.72 & 97.3 & 18.7 & 3.14 & 5.2 & 2.40 & 28.8 \\
%        8 & $\qquad$+ 2-stage training & 3.47 M & 3.06 & 98.2 & 19.8 & 3.21 & 4.2 & 2.40 & 54.3 \\
%        \hline
%        9 & proposed (v1) & 2.92 M &  &  &  &  &  &  & \\
%        10 & $\quad$+ 2-stage training & 2.92 M & 2.98 & 98.2 & \underline{21.1} & 3.22 & 4.1 & 2.80 & 24.9 \\
%        11 & proposed (v2) & 2.53 M & 3.05 & \underline{98.3} & 20.4 & 3.21 & 4.2 & \underline{2.89} & 15.6 \\
%        12 & $\quad$+ 2-stage training & 2.53 M & 2.94 & 97.9 & 18.8 & \textbf{3.23} & 4.6 & \textbf{2.96} & 12.1 \\
        \bottomrule
    \end{tabular}%
    }
    \vspace{-8pt}
\end{table*}

==> table/db.tex <==
\begin{table}
    \setstretch{0.92}
    \captionsetup{labelfont=bf}
    \caption{Information of the datasets. 
    ``\#Ch'' denotes the number of microphone channels.
    ``(Sim)'' and ``(Real)'' denote the synthetic and recorded data. 
    ``(A)'' and ``(R)'' represent anechoic and reverberant.}
    \label{tab:corpora}
    \centering
    \resizebox{1.0\linewidth}{!}{%
        \begin{tabular}{l|ccc} 
        \toprule
        \textbf{Dataset} & \textbf{Hours (train\,/\,dev\,/\,test)}  & \textbf{\mathsymbol{SF}} & \textbf{\#Ch}  \\
        \midrule
        \href{https://datashare.ed.ac.uk/handle/10283/2791}{VoiceBank+DEMAND}~\cite{Speech-Valentini-Botinhao2016} & 8.8\,\textbf{/}\,0.6\,\textbf{/}\,0.6 & 48 kHz & 1\\
        \href{https://github.com/microsoft/DNS-Challenge/tree/interspeech2020/master}{DNS1} (v1)~\cite{DNS_INTERSPEECH2020-Reddy2020} & (A)90\,\textbf{/}\,(A)10\,\textbf{/}\,(R)0.42\,\&\,(A)0.42 & 16 kHz & 1 \\
        \href{http://spandh.dcs.shef.ac.uk/chime\_challenge/chime2016/}{CHiME-4}~\cite{CHiME4-Vincent2017} & (Sim)14.7\,\textbf{/}\,(Sim)2.9\,\textbf{/}\,(Sim)2.3\,\&\,(Real)2.2 & 16 kHz & 5\\
        \href{https://reverb2014.dereverberation.com}{REVERB}~\cite{REVERB-Kinoshita2013} & (Sim)15.5\,\textbf{/}\,(Sim)3.2\,\textbf{/}\,(Sim)4.8\,\&\,(Real)0.7 & 16 kHz & 8\\
        
        \cellcolor[HTML]{EEEEEE} & \cellcolor[HTML]{EEEEEE}(R)58.0\,\textbf{/}\,(R)14.7\,\textbf{/}\,(R)9.0 & \cellcolor[HTML]{EEEEEE} & \cellcolor[HTML]{EEEEEE} \\
        \cellcolor[HTML]{EEEEEE}\multirow{-2}{*}{\href{https://wham.whisper.ai}{WHAMR!}~\cite{WHAMR-Maciejewski2019}} & \cellcolor[HTML]{EEEEEE}(A)58.0\,\textbf{/}\,(A)14.7\,\textbf{/}\,(A)9.0 & \cellcolor[HTML]{EEEEEE}\multirow{-2}{*}{16 kHz} & \cellcolor[HTML]{EEEEEE}\multirow{-2}{*}{2} \\
       \bottomrule
       \end{tabular}%
    }
    % \vspace{-1.7em}
\end{table}

==> table/univ.tex <==
% \begin{table*}
%     \setstretch{0.9}
%     \caption{Speech enhancement performance of the proposed model in diverse conditions. The models are trained only on 8 kHz data (via downsampling), and tested with the original sampling frequencies. ``USES'', ``excl'', ``U2-S'', and ``USES2-Comp'' denote the SE model proposed in~\cite{Toward-Zhang2023}, corpus-exclusive SE, \protect\mathsymbol{USES2-Swin} (proposed), and \protect\mathsymbol{USES2-Comp} (proposed)\protect\hyperlink{footnote:7}{$^7$}. We follow the same training and evaluation configurations as in~\cite{Toward-Zhang2023} to make the results comparable. The DNS1 (reverb) test set can be viewed as an unseen mismatched condition, as the DNS1 training data only contain anechoic samples. The best and second best results are made \textbf{bold} and \underline{underlined}, respectively.}
%     \label{tab:exp_universal}
%     \centering
%     % reduce the distance between columns in a table
%     \setlength{\tabcolsep}{3pt}
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{lc cccc cccc cccc cccc cccc}
%   \toprule
%   & &
%   \multicolumn{4}{c}{\cellcolor[HTML]{EEEEEE}\textbf{PESQ-WB $\uparrow$}} &
%   \multicolumn{4}{c}{\textbf{STOI ($\times100$) $\uparrow$}} &
%   \multicolumn{4}{c}{\cellcolor[HTML]{EEEEEE}\textbf{SDR (dB) $\uparrow$}} &
%   \multicolumn{4}{c}{\textbf{DNSMOS OVRL $\uparrow$}} &
%   \multicolumn{4}{c}{\cellcolor[HTML]{EEEEEE}\textbf{WER (\%) $\downarrow$}} \\
% \multirow{-2}{*}{\textbf{Test set}} &
%   \multirow{-2}{*}{\textbf{Condition}} &
%   \cellcolor[HTML]{EEEEEE}\textbf{USES} &
%   \cellcolor[HTML]{EEEEEE}\textbf{excl} &
%   \cellcolor[HTML]{EEEEEE}\textbf{USES2-Comp} &
%   \cellcolor[HTML]{EEEEEE}\textbf{U2-S} &
%   \textbf{USES} &
%   \textbf{excl} &
%   \textbf{USES2-Comp} &
%   \textbf{U2-S} &
%   \cellcolor[HTML]{EEEEEE}\textbf{USES} &
%   \cellcolor[HTML]{EEEEEE}\textbf{excl} &
%   \cellcolor[HTML]{EEEEEE}\textbf{USES2-Comp} &
%   \cellcolor[HTML]{EEEEEE}\textbf{U2-S} &
%   \textbf{USES} &
%   \textbf{excl} &
%   \textbf{USES2-Comp} &
%   \textbf{U2-S} &
%   \cellcolor[HTML]{EEEEEE}\textbf{USES} &
%   \cellcolor[HTML]{EEEEEE}\textbf{excl} &
%   \cellcolor[HTML]{EEEEEE}\textbf{USES2-Comp} &
%   \cellcolor[HTML]{EEEEEE}\textbf{U2-S} \\
%   \hline
% VoiceBank+DEMAND &
%   1ch, 48kHz &
%   \cellcolor[HTML]{EEEEEE}- &
%   \cellcolor[HTML]{EEEEEE}- &
%   \cellcolor[HTML]{EEEEEE}- &
%   \cellcolor[HTML]{EEEEEE}- &
%   \underline{93.1} &
%   93.0 &
%   \textbf{93.2} &
%   93.0 &
%   \cellcolor[HTML]{EEEEEE}\textbf{11.0} &
%   \cellcolor[HTML]{EEEEEE}10.2 &
%   \cellcolor[HTML]{EEEEEE}10.4 &
%   \cellcolor[HTML]{EEEEEE}\underline{10.8} &
%   \textbf{3.14} &
%   \underline{3.08} &
%   3.02 &
%   3.00 &
%   \cellcolor[HTML]{EEEEEE}\underline{3.2} &
%   \cellcolor[HTML]{EEEEEE}3.6 &
%   \cellcolor[HTML]{EEEEEE}\textbf{2.9} &
%   \cellcolor[HTML]{EEEEEE}3.5 \\
% VoiceBank+DEMAND &
%   1ch, 16kHz &
%   \cellcolor[HTML]{EEEEEE}\textbf{3.11} &
%   \cellcolor[HTML]{EEEEEE}\underline{2.94} &
%   \cellcolor[HTML]{EEEEEE}2.75 &
%   \cellcolor[HTML]{EEEEEE}2.74 &
%   95.0 &
%   \underline{95.1} &
%   \textbf{95.3} &
%   94.7 &
%   \cellcolor[HTML]{EEEEEE}\underline{21.5} &
%   \cellcolor[HTML]{EEEEEE}19.6 &
%   \cellcolor[HTML]{EEEEEE}21.1 &
%   \cellcolor[HTML]{EEEEEE}\textbf{22.0} &
%   \textbf{3.19} &
%   3.13 &
%   3.14 &
%   \underline{3.15} &
%   \cellcolor[HTML]{EEEEEE}3.1 &
%   \cellcolor[HTML]{EEEEEE}\textbf{2.6} &
%   \cellcolor[HTML]{EEEEEE}\textbf{2.6} &
%   \cellcolor[HTML]{EEEEEE}\underline{2.9} \\
% DNS1 (w/o reverb) &
%   1ch, 16kHz &
%   \cellcolor[HTML]{EEEEEE}\textbf{3.23} &
%   \cellcolor[HTML]{EEEEEE}3.03 &
%   \cellcolor[HTML]{EEEEEE}\underline{3.08} &
%   \cellcolor[HTML]{EEEEEE}2.80 &
%   \textbf{97.8} &
%   97.0 &
%   \underline{97.7} &
%   96.9 &
%   \cellcolor[HTML]{EEEEEE}\textbf{19.6} &
%   \cellcolor[HTML]{EEEEEE}\underline{19.3} &
%   \cellcolor[HTML]{EEEEEE}18.9 &
%   \cellcolor[HTML]{EEEEEE}18.7 &
%   \underline{3.32} &
%   \textbf{3.34} &
%   3.28 &
%   3.26 &
%   \cellcolor[HTML]{EEEEEE}\underline{6.4} &
%   \cellcolor[HTML]{EEEEEE}6.9 &
%   \cellcolor[HTML]{EEEEEE}\textbf{5.1} &
%   \cellcolor[HTML]{EEEEEE}7.5 \\
% DNS1 (reverb) &
%   1ch, 16kHz &
%   \cellcolor[HTML]{EEEEEE}\underline{2.75} &
%   \cellcolor[HTML]{EEEEEE}1.86 &
%   \cellcolor[HTML]{EEEEEE}\textbf{2.82} &
%   \cellcolor[HTML]{EEEEEE}1.75 &
%   \underline{89.9} &
%   69.3 &
%   \textbf{90.7} &
%   79.0 &
%   \cellcolor[HTML]{EEEEEE}\underline{13.4} &
%   \cellcolor[HTML]{EEEEEE}5.2 &
%   \cellcolor[HTML]{EEEEEE}\textbf{13.5} &
%   \cellcolor[HTML]{EEEEEE}7.6 &
%   \underline{2.36} &
%   2.23 &
%   2.32 &
%   \textbf{2.55} &
%   \cellcolor[HTML]{EEEEEE}\textbf{28.9} &
%   \cellcolor[HTML]{EEEEEE}60.1 &
%   \cellcolor[HTML]{EEEEEE}\underline{32.7} &
%   \cellcolor[HTML]{EEEEEE}48.0 \\
% CHiME-4 (Simu) &
%   5ch, 16kHz &
%   \cellcolor[HTML]{EEEEEE}2.95 &
%   \cellcolor[HTML]{EEEEEE}\textbf{3.05} &
%   \cellcolor[HTML]{EEEEEE}\underline{3.03} &
%   \cellcolor[HTML]{EEEEEE}2.73 &
%   97.8 &
%   \textbf{98.3} &
%   \underline{98.1} &
%   97.8 &
%   \cellcolor[HTML]{EEEEEE}18.3 &
%   \cellcolor[HTML]{EEEEEE}\textbf{20.4} &
%   \cellcolor[HTML]{EEEEEE}19.1 &
%   \cellcolor[HTML]{EEEEEE}\underline{19.2} &
%   \underline{3.22} &
%   3.21 &
%   \textbf{3.23} &
%   3.14 &
%   \cellcolor[HTML]{EEEEEE}4.4 &
%   \cellcolor[HTML]{EEEEEE}\underline{4.2} &
%   \cellcolor[HTML]{EEEEEE}\textbf{4.1} &
%   \cellcolor[HTML]{EEEEEE}4.4 \\
% REVERB (Simu) &
%   8ch, 16kHz &
%   \cellcolor[HTML]{EEEEEE}2.09 &
%   \cellcolor[HTML]{EEEEEE}1.94 &
%   \cellcolor[HTML]{EEEEEE}\underline{2.10} &
%   \cellcolor[HTML]{EEEEEE}\textbf{2.11} &
%   89.8 &
%   89.0 &
%   \underline{89.9} &
%   \textbf{90.5} &
%   \cellcolor[HTML]{EEEEEE}\textbf{11.9} &
%   \cellcolor[HTML]{EEEEEE}8.8 &
%   \cellcolor[HTML]{EEEEEE}\textbf{11.9} &
%   \cellcolor[HTML]{EEEEEE}\underline{11.8} &
%   \underline{2.98} &
%   2.70 &
%   \textbf{3.00} &
%   2.96 &
%   \cellcolor[HTML]{EEEEEE}\textbf{4.6} &
%   \cellcolor[HTML]{EEEEEE}\underline{4.9} &
%   \cellcolor[HTML]{EEEEEE}\textbf{4.6} &
%   \cellcolor[HTML]{EEEEEE}\textbf{4.6} \\
% WHAMR! (anechoic) &
%   2ch, 16kHz &
%   \cellcolor[HTML]{EEEEEE}\textbf{2.55} &
%   \cellcolor[HTML]{EEEEEE}\underline{2.42} &
%   \cellcolor[HTML]{EEEEEE}\textbf{2.55} &
%   \cellcolor[HTML]{EEEEEE}2.38 &
%   \underline{96.4} &
%   \textbf{96.6} &
%   \underline{96.4} &
%   95.6 &
%   \cellcolor[HTML]{EEEEEE}15.8 &
%   \cellcolor[HTML]{EEEEEE}\textbf{16.1} &
%   \cellcolor[HTML]{EEEEEE}\underline{15.9} &
%   \cellcolor[HTML]{EEEEEE}14.7 &
%   \textbf{3.33} &
%   3.23 &
%   \underline{3.32} &
%   3.26 &
%   \cellcolor[HTML]{EEEEEE}\textbf{6.2} &
%   \cellcolor[HTML]{EEEEEE}\underline{6.3} &
%   \cellcolor[HTML]{EEEEEE}6.4 &
%   \cellcolor[HTML]{EEEEEE}7.6 \\
% WHAMR! (reverb) &
%   2ch, 16kHz &
%   \cellcolor[HTML]{EEEEEE}\textbf{2.51} &
%   \cellcolor[HTML]{EEEEEE}1.72 &
%   \cellcolor[HTML]{EEEEEE}\textbf{2.51} &
%   \cellcolor[HTML]{EEEEEE}\underline{1.91} &
%   \textbf{96.0} &
%   88.7 &
%   \textbf{96.0} &
%   \underline{92.5} &
%   \cellcolor[HTML]{EEEEEE}\textbf{13.8} &
%   \cellcolor[HTML]{EEEEEE}10.3 &
%   \cellcolor[HTML]{EEEEEE}\textbf{13.8} &
%   \cellcolor[HTML]{EEEEEE}\underline{11.4} &
%   \textbf{3.32} &
%   3.00 &
%   \textbf{3.32} &
%   \underline{3.21} &
%   \cellcolor[HTML]{EEEEEE}\textbf{6.5} &
%   \cellcolor[HTML]{EEEEEE}\underline{6.7} &
%   \cellcolor[HTML]{EEEEEE}7.1 &
%   \cellcolor[HTML]{EEEEEE}7.3 \\
%   \hline
% \textbf{Average} &
%   mixed &
%   \cellcolor[HTML]{EEEEEE}\textbf{2.55} &
%   \cellcolor[HTML]{EEEEEE}2.24 &
%   \cellcolor[HTML]{EEEEEE}\underline{2.53} &
%   \cellcolor[HTML]{EEEEEE}2.26 &
%   \underline{94.8} &
%   92.6 &
%   \textbf{94.9} &
%   93.6 &
%   \cellcolor[HTML]{EEEEEE}\textbf{14.9} &
%   \cellcolor[HTML]{EEEEEE}13.4 &
%   \cellcolor[HTML]{EEEEEE}\textbf{14.9} &
%   \cellcolor[HTML]{EEEEEE}\underline{14.0} &
%   \textbf{3.21} &
%   3.04 &
%   \underline{3.20} &
%   3.14 &
%   \cellcolor[HTML]{EEEEEE}\textbf{6.1} &
%   \cellcolor[HTML]{EEEEEE}7.0 &
%   \cellcolor[HTML]{EEEEEE}\underline{6.3} &
%   \cellcolor[HTML]{EEEEEE}7.2 \\
%   \bottomrule
% \end{tabular}%
% }
% \vspace{-1.5em}
% \end{table*}


\begin{table*}
    \setstretch{0.9}
    \caption{Speech enhancement performance of the proposed model in diverse conditions. The models are trained only on 8 kHz data (via downsampling), and tested with the original sampling frequencies. ``USES'', ``excl'', and ``USES2-Comp'' denote the SE model proposed in~\cite{Toward-Zhang2023}, corpus-exclusive SE, and the proposed \protect\mathsymbol{USES2-Comp} model\protect\hyperlink{footnote:7}{$^7$}. We follow the same training and evaluation configurations as in~\cite{Toward-Zhang2023} to make the results comparable. The best and second best results are made \textbf{bold} and \underline{underlined}, respectively.}
    \label{tab:exp_universal}
    \centering
    % The DNS1 (reverb) test set can be viewed as an unseen mismatched condition, as the DNS1 training data only contain anechoic samples.
    % reduce the distance between columns in a table
    \setlength{\tabcolsep}{3pt}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lc ccc ccc ccc ccc ccc}
  \toprule
  & &
  \multicolumn{3}{c}{\cellcolor[HTML]{EEEEEE}\textbf{PESQ-WB $\uparrow$}} &
  \multicolumn{3}{c}{\textbf{STOI ($\times100$) $\uparrow$}} &
  \multicolumn{3}{c}{\cellcolor[HTML]{EEEEEE}\textbf{SDR (dB) $\uparrow$}} &
  \multicolumn{3}{c}{\textbf{DNSMOS OVRL $\uparrow$}} &
  \multicolumn{3}{c}{\cellcolor[HTML]{EEEEEE}\textbf{WER (\%) $\downarrow$}} \\
\multirow{-2}{*}{\textbf{Test set}} &
  \multirow{-2}{*}{\textbf{Condition}} &
  \cellcolor[HTML]{EEEEEE}\textbf{USES} &
  \cellcolor[HTML]{EEEEEE}\textbf{excl} &
  \cellcolor[HTML]{EEEEEE}\textbf{USES2-Comp} &
  \textbf{USES} &
  \textbf{excl} &
  \textbf{USES2-Comp} &
  \cellcolor[HTML]{EEEEEE}\textbf{USES} &
  \cellcolor[HTML]{EEEEEE}\textbf{excl} &
  \cellcolor[HTML]{EEEEEE}\textbf{USES2-Comp} &
  \textbf{USES} &
  \textbf{excl} &
  \textbf{USES2-Comp} &
  \cellcolor[HTML]{EEEEEE}\textbf{USES} &
  \cellcolor[HTML]{EEEEEE}\textbf{excl} &
  \cellcolor[HTML]{EEEEEE}\textbf{USES2-Comp} \\
  \hline
VoiceBank+DEMAND &
  1ch, 48kHz &
  \cellcolor[HTML]{EEEEEE}- &
  \cellcolor[HTML]{EEEEEE}- &
  \cellcolor[HTML]{EEEEEE}- &
  \underline{93.1} &
  93.0 &
  \textbf{93.2} &
  \cellcolor[HTML]{EEEEEE}\textbf{11.0} &
  \cellcolor[HTML]{EEEEEE}10.2 &
  \cellcolor[HTML]{EEEEEE}\underline{10.4} &
  \textbf{3.14} &
  \underline{3.08} &
  3.02 &
  \cellcolor[HTML]{EEEEEE}\underline{3.2} &
  \cellcolor[HTML]{EEEEEE}3.6 &
  \cellcolor[HTML]{EEEEEE}\textbf{2.9} \\
VoiceBank+DEMAND &
  1ch, 16kHz &
  \cellcolor[HTML]{EEEEEE}\textbf{3.11} &
  \cellcolor[HTML]{EEEEEE}\underline{2.94} &
  \cellcolor[HTML]{EEEEEE}2.75 &
  95.0 &
  \underline{95.1} &
  \textbf{95.3} &
  \cellcolor[HTML]{EEEEEE}\underline{21.5} &
  \cellcolor[HTML]{EEEEEE}19.6 &
  \cellcolor[HTML]{EEEEEE}\underline{21.1} &
  \textbf{3.19} &
  3.13 &
  \underline{3.14} &
  \cellcolor[HTML]{EEEEEE}\underline{3.1} &
  \cellcolor[HTML]{EEEEEE}\textbf{2.6} &
  \cellcolor[HTML]{EEEEEE}\textbf{2.6} \\
DNS1 (w/o reverb) &
  1ch, 16kHz &
  \cellcolor[HTML]{EEEEEE}\textbf{3.23} &
  \cellcolor[HTML]{EEEEEE}3.03 &
  \cellcolor[HTML]{EEEEEE}\underline{3.08} &
  \textbf{97.8} &
  97.0 &
  \underline{97.7} &
  \cellcolor[HTML]{EEEEEE}\textbf{19.6} &
  \cellcolor[HTML]{EEEEEE}\underline{19.3} &
  \cellcolor[HTML]{EEEEEE}18.9 &
  \underline{3.32} &
  \textbf{3.34} &
  3.28 &
  \cellcolor[HTML]{EEEEEE}\underline{6.4} &
  \cellcolor[HTML]{EEEEEE}6.9 &
  \cellcolor[HTML]{EEEEEE}\textbf{5.1} \\
DNS1 (reverb) &
  1ch, 16kHz &
  \cellcolor[HTML]{EEEEEE}\underline{2.75} &
  \cellcolor[HTML]{EEEEEE}1.86 &
  \cellcolor[HTML]{EEEEEE}\textbf{2.82} &
  \underline{89.9} &
  69.3 &
  \textbf{90.7} &
  \cellcolor[HTML]{EEEEEE}\underline{13.4} &
  \cellcolor[HTML]{EEEEEE}5.2 &
  \cellcolor[HTML]{EEEEEE}\textbf{13.5} &
  \textbf{2.36} &
  2.23 &
  \underline{2.32} &
  \cellcolor[HTML]{EEEEEE}\textbf{28.9} &
  \cellcolor[HTML]{EEEEEE}60.1 &
  \cellcolor[HTML]{EEEEEE}\underline{32.7} \\
CHiME-4 (Simu) &
  5ch, 16kHz &
  \cellcolor[HTML]{EEEEEE}2.95 &
  \cellcolor[HTML]{EEEEEE}\textbf{3.05} &
  \cellcolor[HTML]{EEEEEE}\underline{3.03} &
  97.8 &
  \textbf{98.3} &
  \underline{98.1} &
  \cellcolor[HTML]{EEEEEE}18.3 &
  \cellcolor[HTML]{EEEEEE}\textbf{20.4} &
  \cellcolor[HTML]{EEEEEE}\underline{19.1} &
  \underline{3.22} &
  3.21 &
  \textbf{3.23} &
  \cellcolor[HTML]{EEEEEE}4.4 &
  \cellcolor[HTML]{EEEEEE}\underline{4.2} &
  \cellcolor[HTML]{EEEEEE}\textbf{4.1} \\
REVERB (Simu) &
  8ch, 16kHz &
  \cellcolor[HTML]{EEEEEE}\underline{2.09} &
  \cellcolor[HTML]{EEEEEE}1.94 &
  \cellcolor[HTML]{EEEEEE}\textbf{2.10} &
  \underline{89.8} &
  89.0 &
  \textbf{89.9} &
  \cellcolor[HTML]{EEEEEE}\textbf{11.9} &
  \cellcolor[HTML]{EEEEEE}\underline{8.8} &
  \cellcolor[HTML]{EEEEEE}\textbf{11.9} &
  \underline{2.98} &
  2.70 &
  \textbf{3.00} &
  \cellcolor[HTML]{EEEEEE}\textbf{4.6} &
  \cellcolor[HTML]{EEEEEE}\underline{4.9} &
  \cellcolor[HTML]{EEEEEE}\textbf{4.6} \\
WHAMR! (anechoic) &
  2ch, 16kHz &
  \cellcolor[HTML]{EEEEEE}\textbf{2.55} &
  \cellcolor[HTML]{EEEEEE}\underline{2.42} &
  \cellcolor[HTML]{EEEEEE}\textbf{2.55} &
  \underline{96.4} &
  \textbf{96.6} &
  \underline{96.4} &
  \cellcolor[HTML]{EEEEEE}15.8 &
  \cellcolor[HTML]{EEEEEE}\textbf{16.1} &
  \cellcolor[HTML]{EEEEEE}\underline{15.9} &
  \textbf{3.33} &
  3.23 &
  \underline{3.32} &
  \cellcolor[HTML]{EEEEEE}\textbf{6.2} &
  \cellcolor[HTML]{EEEEEE}\underline{6.3} &
  \cellcolor[HTML]{EEEEEE}6.4 \\
WHAMR! (reverb) &
  2ch, 16kHz &
  \cellcolor[HTML]{EEEEEE}\textbf{2.51} &
  \cellcolor[HTML]{EEEEEE}\underline{1.72} &
  \cellcolor[HTML]{EEEEEE}\textbf{2.51} &
  \textbf{96.0} &
  \underline{88.7} &
  \textbf{96.0} &
  \cellcolor[HTML]{EEEEEE}\textbf{13.8} &
  \cellcolor[HTML]{EEEEEE}\underline{10.3} &
  \cellcolor[HTML]{EEEEEE}\textbf{13.8} &
  \textbf{3.32} &
  \underline{3.00} &
  \textbf{3.32} &
  \cellcolor[HTML]{EEEEEE}\textbf{6.5} &
  \cellcolor[HTML]{EEEEEE}\underline{6.7} &
  \cellcolor[HTML]{EEEEEE}7.1 \\
  \hdashline
\textbf{Average (Simu)} &
  mixed &
  \cellcolor[HTML]{EEEEEE}\textbf{2.55} &
  \cellcolor[HTML]{EEEEEE}2.24 &
  \cellcolor[HTML]{EEEEEE}\underline{2.53} &
  \underline{94.8} &
  92.6 &
  \textbf{94.9} &
  \cellcolor[HTML]{EEEEEE}\textbf{14.9} &
  \cellcolor[HTML]{EEEEEE}\underline{13.4} &
  \cellcolor[HTML]{EEEEEE}\textbf{14.9} &
  \textbf{3.21} &
  3.04 &
  \underline{3.20} &
  \cellcolor[HTML]{EEEEEE}\textbf{6.1} &
  \cellcolor[HTML]{EEEEEE}7.0 &
  \cellcolor[HTML]{EEEEEE}\underline{6.3} \\
  \hline
CHiME-4 (Real) &
  5ch, 16kHz &
  \cellcolor[HTML]{EEEEEE}- &
  \cellcolor[HTML]{EEEEEE}- &
  \cellcolor[HTML]{EEEEEE}- &
  - &
  - &
  - &
  \cellcolor[HTML]{EEEEEE}- &
  \cellcolor[HTML]{EEEEEE}- &
  \cellcolor[HTML]{EEEEEE}- &
  1.58 &
  \underline{2.96} &
  \textbf{3.08} &
  \cellcolor[HTML]{EEEEEE}85.9 &
  \cellcolor[HTML]{EEEEEE}\underline{12.1} &
  \cellcolor[HTML]{EEEEEE}\textbf{10.3} \\
REVERB (Real) &
  8ch, 16kHz &
  \cellcolor[HTML]{EEEEEE}- &
  \cellcolor[HTML]{EEEEEE}- &
  \cellcolor[HTML]{EEEEEE}- &
  - &
  - &
  - &
  \cellcolor[HTML]{EEEEEE}- &
  \cellcolor[HTML]{EEEEEE}- &
  \cellcolor[HTML]{EEEEEE}- &
  \textbf{3.11} &
  2.10 &
  \underline{3.07} &
  \cellcolor[HTML]{EEEEEE}\underline{5.1} &
  \cellcolor[HTML]{EEEEEE}\textbf{4.9} &
  \cellcolor[HTML]{EEEEEE}\underline{5.1} \\
AMI SDM (Real) &
  1ch, 16kHz &
  \cellcolor[HTML]{EEEEEE}- &
  \cellcolor[HTML]{EEEEEE}- &
  \cellcolor[HTML]{EEEEEE}- &
  - &
  - &
  - &
  \cellcolor[HTML]{EEEEEE}- &
  \cellcolor[HTML]{EEEEEE}- &
  \cellcolor[HTML]{EEEEEE}- &
  2.30 &
  - &
  2.26 &
  \cellcolor[HTML]{EEEEEE}42.5 &
  \cellcolor[HTML]{EEEEEE}- &
  \cellcolor[HTML]{EEEEEE}41.4 \\
AMI MDM (Real) &
  8ch, 16kHz &
  \cellcolor[HTML]{EEEEEE}- &
  \cellcolor[HTML]{EEEEEE}- &
  \cellcolor[HTML]{EEEEEE}- &
  - &
  - &
  - &
  \cellcolor[HTML]{EEEEEE}- &
  \cellcolor[HTML]{EEEEEE}- &
  \cellcolor[HTML]{EEEEEE}- &
  2.36 &
  - &
  2.32 &
  \cellcolor[HTML]{EEEEEE}34.6 &
  \cellcolor[HTML]{EEEEEE}- &
  \cellcolor[HTML]{EEEEEE}34.8 \\
  \hdashline
\textbf{Average (Real)} &
  mixed &
  \cellcolor[HTML]{EEEEEE}- &
  \cellcolor[HTML]{EEEEEE}- &
  \cellcolor[HTML]{EEEEEE}- &
  - &
  - &
  - &
  \cellcolor[HTML]{EEEEEE}- &
  \cellcolor[HTML]{EEEEEE}- &
  \cellcolor[HTML]{EEEEEE}- &
   &
   &
   &
  \cellcolor[HTML]{EEEEEE} &
  \cellcolor[HTML]{EEEEEE} &
  \cellcolor[HTML]{EEEEEE} \\
  \bottomrule
\end{tabular}%
}
\vspace{-1.5em}
\end{table*}
